AI Radiologist: Revolutionizing Liver Tissue Segmentation with Convolutional Neural Networks and a Clinician-Friendly GUI

Artificial Intelligence (AI) is a pervasive research topic, permeating various sectors and applications. In this study, we harness the power of AI, specifically convolutional neural networks (ConvNets), for segmenting liver tissues. It also focuses on developing a user-friendly graphical user interface (GUI) tool, "AI Radiologist", enabling clinicians to effectively delineate different liver tissues (parenchyma, tumors, and vessels), thereby saving lives. This endeavor bridges the gap between academic research and practical, industrial applications. The GUI is a single-page application and is designed using the PyQt5 Python framework. The offline-available AI Radiologist resorts to three ConvNet models trained to segment all liver tissues. With respect to the Dice metric, the best liver ConvNet scores 98.16%, the best tumor ConvNet scores 65.95%, and the best vessel ConvNet scores 51.94%. It outputs 2D slices of the liver, tumors, and vessels, along with 3D interpolations in .obj and .mtl formats, which can be visualized/printed using any 3D-compatible software. Thus, the AI Radiologist offers a convenient tool for clinicians to perform liver tissue segmentation and 3D interpolation employing state-of-the-art models for tissues segmentation. With the provided capacity to select the volumes and pre-trained models, the clinicians can leave the rest to the AI Radiologist.

==> LR_summary.tex <==
\begin{tabular}{
>{\centering\arraybackslash}m{0.02\textwidth} 
m{0.08\textwidth}
>{\centering\arraybackslash}m{0.08\textwidth}
m{0.15\textwidth}
>{\centering\arraybackslash}m{0.1\textwidth}
>{\centering\arraybackslash}m{0.06\textwidth}
>{\centering\arraybackslash}m{0.08\textwidth}
m{0.25\textwidth}
}
\toprule
Ref.                        & \multicolumn{1}{c}{Abbrv.} & Platform           & \multicolumn{1}{c}{GUI Framework}   & ML usage & Organ                  & Auto       & \multicolumn{1}{c}{Functionality}                                                     \\
\midrule
\cite{Arthurs2021}          & CRIMSON                    & Desktop            & MITK + PyQt                         & No       & Vessels                & No         & Generates 3D haemodynamics studies                                                 \\
\cite{Berg2019}             & ilastik                    & Desktop            & PyQt                                & Yes      & Cell Nuclei            & Yes        & Interactive software to segment, classify, track, and count cells                     \\
\cite{Yushkevich2019}       & ITK-SNAP                   & Desktop            & Qt + FLTK                           & Yes      & Generic                & Semi       & New features addition to ITK-SNAP tool   \\
\cite{Kordt2018}            & N/A                        & Web                & VISIAN                              & No       & Brain                  & Semi       & Interactive segmentation for brain tumor              \\
\cite{Arganda-Carreras2017} & TWS                        & Desktop            & Plugin in Fiji                      & Yes      & Cells                  & Yes        & A plugin in Fiji framework to add WEKA initiative    \\
\cite{Aleem2020}            & N/A                        & Web                & React + Material UI                 & Yes      & Lungs                  & Yes        & COVID-19 case testing over lungs                                                      \\
\cite{Yang2020}             & NuSeT                      & Desktop            & Tkinter                             & Yes      & Cell Nuclei            & Yes        & Automated training on and segmentation of nuclei cells using AI                          \\
\cite{Kim2020}              & N/A                        & Web                & HTML + CSS + JavaScript + Bootstrap & Yes      & Spine                  & Yes        & Spine segmentation web application using U-Net ConvNet                                \\
\cite{Calisto2021}          & Breast\-Screening            & Web                & HTML + jQuery (JavaScript)          & Yes      & Breast                 & Yes        & AI utilization in breast images cancer classification                                 \\
\cite{Song2020}             & FAE                        & Desktop            & PyQt                                & Yes      & Pancreas               & Yes        & Prostate cancer classical ML classifier with engineered features     \\
\cite{Chheang2021}          & N/A                        & Desktop Web Server & Unity + VRTK + Photon               & No       & Liver                  & No         & VR for liver's tumors resection                                                       \\
\cite{Trestioreanu2018}     & N/A                        & Desktop            & Unity + HoloLens                    & Yes      & Liver                  & Yes        & Liver \& tumors segmentation with AR capabilities                                     \\
\cite{Chen2019deep}         & DeepLNAnno                 & Web                & Not Disclosed                       & Yes      & Lungs                  & Semi       & Lung nodules annotating system over CT-based images                                   \\
\cite{Yayuan2021}           & RadCloud                   & Web/\-Mobile         & Not Disclosed                       & Yes      & Generic                & Yes        & Facilitate access for AI-assisted research for different challenges \\
\bottomrule
\end{tabular}
